High Information Density and Low Coverage Data Storage in DNA with Efficient Channel Coding Schemes

DNA-based data storage has been attracting significant attention due to its extremely high data storage density, low power consumption, and long duration compared to conventional data storage media. Despite the recent advancements in DNA data storage technology, significant challenges remain. In particular, various types of errors can occur during the processes of DNA synthesis, storage, and sequencing, including substitution errors, insertion errors, and deletion errors. Furthermore, the entire oligo may be lost. In this work, we report a DNA-based data storage architecture that incorporates efficient channel coding schemes, including different types of error-correcting codes (ECCs) and constrained codes, for both the inner coding and outer coding for the DNA data storage channel. We also carried out large scale experiments to validate our proposed DNA-based data storage architecture. Specifically, 1.61 and 1.69 MB data were encoded into 30,000 oligos each, with information densities of 1.731 and 1.815, respectively. It has been found that the stored information can be fully recovered without any error at average coverages of 4.5 and 6.0, respectively. This experiment achieved the highest net information density and lowest coverage among existing DNA-based data storage experiments (with standard DNA), with data recovery rates and coverage approaching theoretical optima.

==> Inner-code.tex <==
\section{Efficient Design of Inner Codes}

\subsection{Objectives and Design Outline}

To improve the reliability of DNA storage, our broad objective for designing the inner codes is to provide {\em practical quaternary codes} that achieve {\em high information rate} with novel encoding and decoding schemes, {\em offering error-correction capability with only a small number of coverage}. Our main contribution is an efficient combination of constrained codes with error-correction codes (ECCs). While constrained codes can significantly reduce the occurrence of errors in a DNA storage system, such codes themselves cannot correct errors, and hence, the design of optimized ECCs plays an important role in recovering the DNA sequences whenever errors occur. 
\vspace{1mm}

Firstly, to obtain practical codes, we use constrained coding to guarantee that all DNA encoded sequences satisfy two crucial biochemical constraints in a DNA storage channel, that are {\em runlength limited constraint} (that restricts a long run of identical symbols) and {\em GC-content constraint} (that controls the appearance of nucleotides G and C) \cite{exp1, yazdi:2015, ttdna:2021,Yazdi.2017}. For example, Ross \et{} \cite{ross2013} reported that a
run of more than six identical symbols would result in
a significant increase of substitution and deletion errors (see
\cite{ross2013}, Fig. 5), and therefore, such long runs should be avoided. On the other hand, it was shown that DNA sequences with GC-content that are too high or too low are more prone to both synthesis and sequencing errors \cite{exp1,ttdna:2021,ross2013,P:2006}. Therefore, most literature experiments used DNA
sequences whose GC-content is close to 50\% (for example, between 45\% to 55\% in \cite{Yazdi.2017}, or between 40\% to 60\% in \cite{exp1}). In this work, at the first step of designing inner codes (Step I: the constrained coding step), we restrict the maximum run of identical symbols to be at most three and the GC-content to be within 45\% to 55\%. After that, all output codewords will proceed to the final step (Step II: the error-correction coding step), where additional redundancy is generated to enhance the error-correction capability. 
\vspace{1mm}

The efficiency of Step II plays an important role in obtaining full recovery of original data, and most importantly, with only a small number of coverage. In this project, we design two different ECCs and provide a detailed analysis on the performance of these two codes. The differences in the design of these two codes are highlighted as follows. 
\begin{enumerate}
\item {\em ECC Type A: adapting the single edit correction code}. In this code, the error-correction capability is enforced over every DNA sequence. Particularly, each DNA sequence itself is capable of correcting a single edit error (either a deletion, a substitution, or an insertion), and hence, the decoding procedure is performed over individual sequences. The additional redundancy is 9 symbols per sequence. Through this experimental study, the combination of constrained coding with ECC type A gives the smallest number of coverage (approximately $4.5$). To the best of our knowledge, this is also the smallest number of coverage as compared to all previous experimental studies. 
%During the decoding procedure, the decoder proceeds to decode The additional redundancy is 9 symbols per sequence.
%Here, we adapt the encoding scheme, presented in a companion work \cite{ttdna:2021}, to design such an SEC. The additional redundancy is 9 symbols per sequence. 
\vspace{1mm}

\item  {\em ECC Type B: adapting the single edit reconstruction code}. In this design, we take advantage of a significant DNA storage channel characteristic, that many copies of the same DNA sequences are generated during both synthesis and sequencing processes \cite{yazdi:2015, exp1}, to further reduce the number of redundant bits, or equivalently, increase significantly the information rate. In an ECC type B, the additional redundancy is only two symbols, and hence, such a code obtains a higher information rate than an ECC type A. We overcome the coding challenge when the DNA sequences in an ECC type B have a weaker error-correction capability by performing the decoding procedure over every {\em set of sequences} having the same index, instead of over individual sequences in an ECC type A. In \cite{cai:2021}, we showed that when the coverage is more than five, such an ECC type B can also correct a single edit error, and hence, have the same performance as ECC type A.   
\end{enumerate}



%Particularly, crucial to the second design is the concept of {\em reconstruction code}. In such a design, we take advantage of a significant DNA storage channel characteristic, that many copies of the same DNA sequences are generated during both synthesis and sequencing processes \cite{yazdi:2015, exp1}, to further reduce the number of redundant bits, or equivalently, increase significantly the information rate. The problem of reconstructing a codeword from its several noisy copies is referred to as a sequence reconstruction problem (for example, see \cite{cai:2021,len:DNA1,len:DNA2,sini:DNA}). %The first design, 
%\begin{enumerate}
%\item {\em ECC Type I: single edit correction code (SEC)}. In this code, every DNA codeword is capable of correcting a single error (either a deletion, a substitution, or an insertion). Here, we adapt the encoding scheme, presented in a companion work \cite{ttdna:2021}, to design such an SEC. The additional redundancy is 9 symbols per sequence. 
%\item  {\em ECC Type II: single edit reconstruction code (SRC)}. In this code, the additional redundancy is only two symbols. Consequently, such an SRC has a higher information rate than an SEC. Although the DNA sequences in an SRC have a weaker error-correction capability than those in an SEC, our decoding algorithm for an SRC is performed over every {\em set of sequences} having the same index, instead of over individual sequences in an SEC. In \cite{cai:2021}, we showed that when the coverage is at least five, such an SRC can correct a single edit error, and hence, have the same performance as an SEC.   
%\end{enumerate}

To achieve high information rate codes, in both constrained coding and error-correction coding steps, we propose novel, optimized, and low-complexity encoding and decoding algorithms that incur a sufficiently small amount of redundancy, as compared to other state-of-the-art schemes. Particularly, crucial to our constrained coding is the {\em sequence replacement technique} (SRT), an efficient method for removing forbidden subsequences in a constrained system \cite{srt:1,srt:2,srt:3} (refer to Section III-B for detailed construction).


\subsection{Efficient Constrained Coding Schemes}
%In this section, we present an efficient coding scheme that translates arbitrary data into DNA sequences that satisfy the runlength limited constraint (where the repetition of identical symbols is restricted to be at most three) and the GC-content constraint (the GC-content is restricted to be within $[45\%, 55\%]$). 

We first go through notations. For ease of exposition, we use the decimal alphabet $\Sigma=\{0,1,2,3\}$ to present our coding schemes instead of the the nucleotides $\D=\{{A},{T},{C},{G}\}$. We define the following relation $\Phi$ between the decimal alphabet $\Sigma$ and the nucleotides $\D$ as follows:
 \begin{equation*}
 \Phi: 0 \to {A}, 1 \to {T}, 2 \to {C}, \text{ and } 3 \to {G}.
 \end{equation*}

\begin{definition}
Let $\bsg=\sigma_1\sigma_2\ldots\sigma_n \in\Sigma^n$, denote a quaternary sequence of length $n$. Given $\ell>0$, we say that $\bsg$ is \emph{$\ell$-runlength limited} if any run of the same nucleotide is at most $\ell$. %On the other hand, the ${G}{C}$-content or weight of strand $\bsg$, denoted by $\omega(\bsg)$, is defined by $\omega(\bsg)=(1/n).\sum_{i=1}^n \varphi(\sigma_i)$ where $\varphi(\sigma_i)=0$ if $\sigma_i\in\{0,1\}$ and $\varphi(\sigma_i)=1$ if $\sigma_i\in\{2,3\}$. Given $\epsilon>0$, we say that $\bsg$ is \emph{$\epsilon$-balanced} if $|\omega(\bsg)-0.5|\leq \epsilon$, in other words, $\omega(\bsg) \in [0.5-\epsilon,0.5+\epsilon]$. In particular, when $n$ is even and $\epsilon=0$, we say $\bsg$ is {\em ${\tt G}{\tt C}$-balance}.
\end{definition}

==> Outer-code.tex <==
\section{Outer Code Coding Scheme}
In DNA-based data storage, only a fraction of oligos can be seen during the sequencing due to the unordered storage manner \cite{heckel2019acharacterization}. Therefore, the outer code is necessary to achieve an error-free system at a relatively low coverage. In this section, we illustrate the encoding and decoding processes of the outer code implemented in our experiment. The fountain codes \cite{mackay2005fountain}, originally designed for erasure channel, where an encoded symbol transmitted over the channel is either lost or received with no error, exhibits a rateless property, enabling its integration with constrain code. Thus, prior work \cite{erlich2017dna} employed the Luby transform(LT) codes, recognized as the first practical realization of fountain codes, as the outer code to achieve an efficient architecture.

In our experiment, another class of fountain codes, namely Raptor codes, is adopted as the outer code. Compared to LT codes, Raptor codes achieve better error-correction performance while remains linear encoding and decoding by adding a pre-code. 

\subsection{Encoding} 
In our experiment, we encode 28500 and 28970 binary strings of length 452 and 466 into 30000 strings for scheme 0 and 2, respectively. The first step of Raptor codes encoding involves a high code rate pre-code encoding to generate the redundant strings known to both the sender and receiver. Subsequently, codewords are generated following the encoding scenario of LT codes. At the beginning of each encoding round, a subset of strings is selected randomly. After that, the output codeword is represented by 2 spliced components: the bitwise result of the selected strings and their corresponding seed. The seed is used to infer which strings the output codeword is generated from. Given the output string sizes of 30000, at least $\lfloor \log_{2}30000 \rfloor = 15$ bits is needed for the seed. Notably, some seeds may be unusable due to their corresponding output string don't satisfy the desired homopolymer and GC content constrains. Therefore, an additional bit is appended, resulting in a 16-bits seed, enabling the generation of twice as many candidate codewords. In each round, once the seed is generated, the corresponding quaternary string is derived by replacing $\{00, 01, 10, 11\}$ by $\{$A, T, C, G$\}$, and checked if it pass the homopolymer constrain. 

\subsection{Decoding}
The decoding algorithm for fountains code for erasure channel has been well studied and developed, e.g., structured Gaussian elimination(SGE) is known as the maximum likelihood(ML) decoder that can be performed efficiently. However, the received strands may be erroneous in DNA-based data storage, rendering the SGE decoding algorithm inapplicable. Prior work \cite{erlich2017dna} perform the belief propagation(BP) decoding, which is able to decode fountain codes in noisy channel. Nonetheless, the check nodes of fountain codes are generated in a stochastic manner, thereby resulting in a poor performance of BP decoding. In this experiment, we employ 2 type of decoding schemes for the Raptor codes. Let $\mathbf{R}$ be the input of the outer code decoder and each row of $\mathbf{R}$ be a output codeword by the inner code decoder.

\subsubsection{SGE decoder}
As previously noted, the SGE decoder is specifically designed for the erasure channel, whereas the decoding is very likely to be unsuccessful if any individual erroneous string contributes to the decoding. DNA-based data storage system within its multiple copies feature, facilites the use of the SGE decoder. Intuitively, strings with higher copy numbers are more reliable, as the right strings dominate all the strings. Consequently, the SGE decoding is exclusively performed on the most reliable strings. It could be viewed that the strings within low copy numbers are erased as they are more likely to be errouneous.

\subsubsection{BFA decoder}
Basis-finding algorithm(BFA) \cite{he2023basis} is the state-of-the-art decoding algorithm for decoding fountain codes in noisy channel. The core idea of BFA is to evaluate the reliability of each string by the number of it attends the linear representation of our strings. In our experiment, we slightly modify the BFA to adapt the DNA-based data storage system.

Firstly, we initialize the reliability of each string based on 2 factors: Its copy number. and its hanmming weight(i.e., the number of ones). Secondly, a set of basis $\mathbf{B}$, i.e., a maximum linearly independent subset of $\mathbf{R}$ is found following such scenario: iterate all the strings from the most reliable to the least, add each string into $\mathbf{B}$ if it can not be linearly represented by the strings already in $\mathbf{B}$. After that, the basis is used to linearly represent all the strings that don't form the basis. Finally, the SGE decoding is performed on the basis elements attending the largest numbers of linear representations.
